Bayesian Optimization Meets Hybrid Zero Dynamics: Safe Parameter Learning for Bipedal Locomotion Control

In this paper, we propose a multi-domain control parameter learning framework that combines Bayesian Optimization (BO) and Hybrid Zero Dynamics (HZD) for locomotion control of bipedal robots. We leverage BO to learn the control parameters used in the HZD-based controller. The learning process is firstly deployed in simulation to optimize different control parameters for a large repertoire of gaits. Next, to tackle the discrepancy between the simulation and the real world, the learning process is applied on the physical robot to learn for corrections to the control parameters learned in simulation while also respecting a safety constraint for gait stability. This method empowers an efficient sim-to-real transition with a small number of samples in the real world, and does not require a valid controller to initialize the training in simulation. Our proposed learning framework is experimentally deployed and validated on a bipedal robot Cassie to perform versatile locomotion skills with improved performance on smoothness of walking gaits and reduction of steady-state tracking errors.

==> problem.tex <==
\section{Problem Statement}
\label{sec:Problem}
\subsection{Bi-pedal robot gait regulator}
In this work, we consider the problem of gait regularization of the walking controller for the Cassie robot proposed in \cite{li2020animated}. A desired gait $g_d$ is obtained by interpolating a gait library $G$ comprised of different combinations of the gait parameters $p=\begin{bmatrix}v_x&v_y&h\end{bmatrix}^T$, with respect to the robot's current observed gait parameters  $\hat{p}=\begin{bmatrix}\hat{v}_x&\hat{v}_y&\hat{h}\end{bmatrix}^T$. In order to track the reference gait parameters $p_d$ while maintaining a stable walking gait, a gait regulator is applied to the desired gait, with a correction $\delta_{g_d}$ defined as 
\begin{align}
    \begin{aligned}
    \delta_{g_d}=\begin{bmatrix}\delta_{q_3^{sw}}\\\delta_{q_1^{sw}}\\\delta_{q_4^{st}}\\\end{bmatrix}=K_p(h^d)(p^d-p)+K_D(h^d)(\Dot{p}_d-\Dot{\hat{p}})
    \end{aligned}
\end{align}
where $\delta_{q_{3}^{sw}}$ and $\delta_{q_{1}^{sw}}$ are corrections for the leg pitch and abduction joint of the \textit{swing} leg, and $\delta_{q_{4}^{st}}$ represents the correction to the \textit{stance} leg length. $p_d$ and $\hat{p}$ are the desired and current gait parameters respectively. Thus the commanded gait $g_u$ becomes the sum of the reference gait $g_d$ and regulating term $\delta_{g_d}$,
\begin{align}
    \begin{aligned}
g_u = g_d+\delta_{g_d}
    \end{aligned}
\end{align}
This walking controller has a gain scheduling module where the aforementioned PD gains $K_P$ and $K_D$ are scheduled based on the reference gaits $g_d$. This is achieved by interpolating in a look-up parameter table with respect to $g_d$.
\subsection{Bayesian Optimization}
The goal of Bayesian optimization is to find a set of parameters $a\in A$ in a specified domain $A\in \mathbb{R}^d$


